Exploring the Limits of Large Scale Pre-training

Recent developments in large-scale machine learning suggest that by scaling up data, model size and training time properly, one might observe that improvements in pre-training would transfer favorably to most downstream tasks. In this work, we systematically study this phenomena and establish that, as we increase the upstream accuracy, the performance of downstream tasks saturates. In particular, we investigate more than 4800 experiments on Vision Transformers, MLP-Mixers and ResNets with number of parameters ranging from ten million to ten billion, trained on the largest scale of available image data (JFT, ImageNet21K) and evaluated on more than 20 downstream image recognition tasks. We propose a model for downstream performance that reflects the saturation phenomena and captures the nonlinear relationship in performance of upstream and downstream tasks. Delving deeper to understand the reasons that give rise to these phenomena, we show that the saturation behavior we observe is closely related to the way that representations evolve through the layers of the models. We showcase an even more extreme scenario where performance on upstream and downstream are at odds with each other. That is, to have a better downstream performance, we need to hurt upstream accuracy.

==> Figure_issues.tex <==
Todo
Set up the webpage?
send to some folks?
to check "well below" part

\begin{itemize}
    \item Figure 1: 
%   - y-axis labels are missing
%   - the legend 0.0e0 needs to be removed
%   - are all sizes $a * 10^10$? or does this have to be corrected? 
%   -its not convex hull
    
   \item Figure 2 
%   *pareto frontier* word needs to be removed its not convex hull
   
   \item Figure 3 the word *downstream dataset on top of the plot is misleading, please remove (N/A)
   
   \item Figure 4, if possible please change *err(inf)* to *err_inf* to be aligned with text
   
   \item Figure 8
%   what is US task here? please add to caption (Fixed)
   
   \item Figure 9 
%   the legend for small and mid-size circle is missing, the label for the figure on the right is missing
   
   \item Figure 
%   10 y-axis label is missing
   
    \item Figure 12 
    - y-axis label is missing (Fixed)
    -legend labels are missing  (Fixed)
    
    
   \item Figure 13: 
   - y-axis labels are missing
   - the legend 0.0e0 needs to be removed
   - are all sizes $a * 10^10$? or does this have to be corrected?      

   \item Figure 14 the word *downstream dataset on top of the (Fixed) plot is misleading, please remove
   \item Figure 15 the word  (Fixed) *downstream dataset on top of the plot is misleading, please remove (Fixed)
   \item Figure 16 the word *downstream dataset on top of the plot is misleading, please remove (Fixed)
   
   \item Figure 23, if possible please change *err(inf)* to *err_inf* to be aligned with text (Fixed)
   
   \item Figure 28 is cropped in a weird way and the caption is also cropped. please fix this (Fiixed)
   
   \item Figure 29 is cropped in a weird way  (removed)
   
   \item Figure 31 y-axis label is missing
   
    \item Figure 32 
    -y-axis label is missing, 
    -some part of legend is missing
    
    
    \end{itemize}

==> comments.tex <==

\section{Neil}:
One of the concluding sentences "We assert that we should refrain from focusing on the performance of only one downstream task" I could not agree with more!  I love to see when papers report more than just ImageNet (shameless plug for VTAB ;) ).

There is a lot there, and I only had time so far for a quick skim, but here are some quick comments:

Done 1) First, a boring bureaucratic thing:  IIUC, you present JFT upstream numbers (e.g. Fig 1). There is precedent for this, but IIUC you report *a lot* of JFT numbers. I don't see JFT approval in pubapprove, do you have some offline approval from Tom/Image Understanding for publishing all these raw JFT scores? (I am sure they will be fine with it, but just checking)

Done 2) I am probably misunderstanding something, but I didn't quite follow this line of reasoning: e.g. in the abstract "[...] one can obtain a model that can be used successfully in few-shot settings in most downstream tasks" followed by "we investigate this premise empirically and provide a strong case against it"

I think the literature shows that one *can* obtain a model that performs well on many downstream tasks (e.g. ViT, Mixer, BERT from NLP, etc. all get good scores on many tasks). I think your results show that there are still loads of unsolved challenges (e.g. mismatched US and DS performance), and that any one model is *not optimal* (the best hyperparameter settings are different for different tasks!)  So my takeaway here is that although such models can be good, if we understood better the US/DS relation (which this paper takes steps towards) they could be a whole lot better still!  But "one can obtain a model that can be used successfully in few-shot settings in most downstream tasks" is still true, right?

Done 3) How is saturation defined exactly?

This is something we were thinking about a bit for this paper (very recent, wouldn't expect you to have seen it, or to cite it, since its concurrent). There are 2 ways to think about it
 - All tasks saturate in absolute terms since you can't get better than 100% accuracy, however, a power-law relationship (like in scaling laws) may still apply, and one can get to 0% error eventually with enough compute
 - Henighan et al. (and us) observe saturation even before 0% though, as did we, which indicates that large models will saturate a task faster than a power law.

Just wondering how you think about when a task is "saturated": going from 99% to 99.9% may or may not be useful depending on the task.  (Again I previewed the paper quite fast, so maybe I missed this nuance!)

Done 4) "We note that for datasets such as ImageNet that are close to JFT"

I might avoid subjective statements about what JFT looks like or how it was created. I feel here we need to quantify (how similar is JFT really to ImageNet, how is it scaled, etc.) and get formal approval to release precise statements.

Done "One cannot guarantee that mindlessly increasing upstream data leads to upstream data covering..." Similarly, I know this is a generic statement, but we should be mindful of implying that JFT was created "mindlessly", or at least quantify that statement.

 btw Neil had a few suggestion or improving the paper:
*TODO* 1. Introducing L2 norm as an indicator for how much information is encoded in the model is not necessarily correct. we can soften it by saying it can be correlated or something. 
Done 2. He liked Figure 3 but he said one should ponder a lot to get the coolness of it. He also suggested that we can be summarize the who figure for all DS tasks into  an "additional" single plot where we have a single point in slope of red vs slope of green curve. 
Done 3. He also said he would choose better titles for investigation/observation sections. also these titles are not consistent across sec 2 and 3.



\section{Alex}



\section{papers to read}

We also give evidence for the intuition that “more is better” by showing that representations learnt with (1) more data, (2) bigger width, or (3) more training time can be “plugged in” to weaker models to improve performance. 
https://arxiv.org/pdf/2106.07682.pdf

Scaling up vision transformer


==> post_deadline.tex <==
optimal wd being different for different ds, us we might be able to learn about how to relate other concepts we created to the optimal weight decay.

The optimal weight decay of different DS tasks can be very different, i.e., If we take different DS tasks or the US task into account when tuning the value for this hyper-parameter we will end up with different WD optimums. 
Also, there are cases where increasing or decreasing US head WD results in improved performance for a DS task and degraded performance for another DS task. Therefore, one cannot simply save a checkpoint of a model pre-trained on an upstream task and use it for downstream tasks. 
(Q: can someone load a checkpoint and do a few iterations with a different weight decay on the head instead of retraining from the beginning? If all we are doing is pushing information, we shouldn't need to redo everything for each weight decay on the head, right?)

 gradient of US and DS may become perpendicular. needs a simple loss surface. the examples that are contributing are from the Set3 above. \hscomment{ToDo Mostafa, once the experiment reaches a conclusion}
 
 \begin{itemize}
\item if we can provide a distance measure we can use it to explain this. Can we use the idea in scaling laws for transfer to measure distribution shift \hscomment{delayed}
\item  Look at DS to US plot and see where DS plateaus. Say it is at 80$\%$ on US.Take the model at 90,80,70 and check which parts of US dataset they have learned during these periods of accuracy. Do transfer learning on those US sub-datasets i.e., pre-train on these only and look into DS task performance. When you pre-train, start from an init where the model is already at 70$\%$. 1. Assume we have a training plot similar to Figure~\ref{fig:regions} for the performance in the downstream few-shot in different steps:
\begin{itemize}
\item[1] We take Ckpt1, classify all the examples in the upstream training set and take those that are correctly classified and make Set1. 
\item[2] We then take Ckpt2, classify all the examples in the upstream training set and take those that are correctly classified and drop those that are included in Set1 and make Set2.
\item[3] We then take Ckpt3, classify all the examples in the upstream training set and take those that are correctly classified and drop those that are included in Set1 and Set2 and make Set3.
\item[4] Then we initialize the model with Ckpt1, but train it once with Set2 and once with Set3 (we skip examples in Set2) and check how different the downstream performance will be. \hscomment{delayed}
\end{itemize}
\begin{figure}[ht]
    \centering
    \includegraphics[width=.5\linewidth]{figs/regions.png}
    \caption{\small Regions  
    }
    \label{fig:regions}
\end{figure}

\item did we check which classes of caltech are being misclassified? maybe they are typical in caltech but are rarer in jft. maybe the distribution on classes are different
or visualize the examples that are not being classified well vs examples that are correctly classified. h1. Caltech visualization. exists some stuff in caltech that does not exist in jft,
\item h2. JFT visualization there are some examples in jft that are useless for caltech. take two models that have different acc on jft but same acc on caltech. take two example groups from JFT: both are correct, higher acc one is getting right and lower acc is not getting right


\end{itemize}
